Incorporating Visual Semantics into Sentence Representations within a Grounded Space

Language grounding is an active field aiming at enriching textual representations with visual information. Generally, textual and visual elements are embedded in the same representation space, which implicitly assumes a one-to-one correspondence between modalities. This hypothesis does not hold when representing words, and becomes problematic when used to learn sentence representations --- the focus of this paper --- as a visual scene can be described by a wide variety of sentences. To overcome this limitation, we propose to transfer visual information to textual representations by learning an intermediate representation space: the grounded space. We further propose two new complementary objectives ensuring that (1) sentences associated with the same visual content are close in the grounded space and (2) similarities between related elements are preserved across modalities. We show that this model outperforms the previous state-of-the-art on classification and semantic relatedness tasks.

==> one_sentence.tex <==
\newlength{\ltwosmall}
\setlength{\ltwosmall}{21pt}

\begin{table*}[t]
\small
    \begin{center}
	%\begin{tabularx}{\textwidth}{l r | C{\ltwosmall} C{\ltwosmall}  C{\ltwosmall} | Y Y Y Y Y}
	\begin{tabularx}{\textwidth}{l r | C{\ltwosmall} C{\ltwosmall} C{\ltwosmall} | Y Y Y Y Y}
    	\multicolumn{1}{r}{} & & \multicolumn{3}{c|}{\textbf{Structural measures}} & \multicolumn{5}{c}{\textbf{Semantic relatedness}} \\
    	
        %& \textit{Concreteness}  & & & & \textit{2.75} & \textit{3.10} & \textit{2.61} & \textit{2.39} & \textit{3.12}\\
    	
    	\multicolumn{2}{c|}{Model} & $\rho_{vis}$ & $C_{intra}$ & $C_{inter}$ & STS/All & STS/Cap. & STS/News &STS/For. & SICK \\
        \hline
Text-only & \textbf{ST}  &16 & 43& 25   & 40/41  & 44/42 & 38/42 & 21/22 &  52/55 \\ 
Projection \textbf{P} & $\textbf{P}^p(0)$ & 35 & 36& 2&58/62& 77/78 & 40/45 & 22/25 & 60/66\\
%Projection \textbf{P}(R) & $\textbf{P}^p(0)$ & \\
        \hline
Cluster $\textbf{M}_{cluster}$ &$ \textbf{M}^p(0,\phantom{.1}0,1)$ & 31&36 &2 &58/61 & 76/77 & 40/45 & 21/23 & 61/66 \\ 
%Cluster $\textbf{M}_{cluster}$ &$ \textbf{M}^p(0,\phantom{.1}0,1)(R)$ &  \\ 
Perceptual $\textbf{M}_{perc}$ & $\textbf{M}^p(0,\phantom{0.}1,0)$ &50 & 43&21 &54/56&68/68&40/44&21/23&58/61\\
%Perceptual $\textbf{M}_{perc}$ & $\textbf{M}^p(0,\phantom{0.}1,0)(R)$ & \\
Both combined $\textbf{M}_{both}$ &  $\textbf{M}^p(0,0.1,1)$ & 39 &40 &3 &57/62 & 75/77 & 40/45 & 22/24 & 60/67 \\ 
%Both combined $\textbf{M}_{both}$ & $\textbf{M}^p(0,0.1,1)(R)$ &\\ 
    \end{tabularx}
    \end{center}
    \vspace{-0.2cm}
    \caption{Two sentences per video}
    \label{onesent}
\end{table*}

==> partial_table.tex <==
\newlength{\lsmallbig}
\setlength{\lsmallbig}{27pt}
\newlength{\lverysmall}
\setlength{\lverysmall}{7.7pt}
\begin{table*}[t]

    \begin{center}
    \footnotesize
	\begin{tabularx}{\textwidth}{ l r | C{\lsmallbig} C{\lsmallbig}  | Y Y Y Y Y Y Y}
	
    	\multicolumn{1}{c}{} & \multicolumn{1}{r|}{}  & \multicolumn{2}{c|}{\textbf{Semantic relatedness}} &  \multicolumn{7}{c}{\textbf{Classification}}\\
    	
    	\multicolumn{2}{c|}{ Model } & {\fontsize{\lverysmall}{0}\selectfont STS} &  {\fontsize{\lverysmall}{0}\selectfont SICK} & {\fontsize{\lverysmall}{0}\selectfont MSRP} & {\fontsize{\lverysmall}{0}\selectfont MPQA} & {\fontsize{\lverysmall}{0}\selectfont MR} & {\fontsize{\lverysmall}{0}\selectfont SUBJ} & {\fontsize{\lverysmall}{0}\selectfont TREC} & {\fontsize{\lverysmall}{0}\selectfont CR} & {\fontsize{\lverysmall}{0}\selectfont SST} \\

    	\hline
\multirow{1}{*}{Text-only} & \textbf{ST} & 40/41  &   52/55  & 71.6 & 86.2 & 75.9 & 92.1 & 89.4 & \textbf{82.5} & 83.3 \\
Sequential & \textbf{SEQ}  &47/44 & 58/69 & 70.0 & 86.1 & 75.8 & 92.2 & 89.2 & 81.9 & 83.3 \\
\multirow{2}{*}{Projection} & $\textbf{P}^{\varnothing}$ &47/48 &56/66&72.8&\textbf{86.3}&76.5 &92.7&89.4&80.4&82.0 \\ 
& $\textbf{P}^p$ & 41/39  & 54/59 & 73.1 & 86.2 & 76.7 & 92.5 & 88.8 & 81.3& 83.7 \\ 
External & \textbf{E}& 43/41 & 51/56 & 72.2 & 86.2 & 76.4 & 92.1 & 88.9 &79.5 & 83.9 \\
\hline
\multirow{2}{*}{Our model} & $\textbf{M}^{\varnothing}$ & \textbf{50}/\textbf{51} & \textbf{60}/\textbf{70} & 72.2 & \textbf{86.3} & \textbf{77.2} & \textbf{93.0} & \textbf{90.4} &81.0 & 82.1\\
& $\textbf{M}^{p}$ & 44/43  & 54/60 & \textbf{74.4} & 86.1 & 76.3 & 92.6 & 88.8 & 81.3& \textbf{84.6} \\  %pas 
    \end{tabularx}
    %\vspace{-0.2cm}
    \caption{(MSVD) Semantic relatedness and classification performances of different models and scenarios.\label{partial_table}}
    \vspace{-0.4cm}
    \end{center}
\end{table*}





==> table_aligning_similarity.tex <==
\newlength{\ltwosmall}
\setlength{\ltwosmall}{21pt}

\begin{table*}[t]
\small
    \begin{center}

	\begin{tabularx}{\textwidth}{l r | C{\ltwosmall} C{\ltwosmall} C{\ltwosmall} | Y Y Y Y Y}
    	\multicolumn{1}{r}{} & & \multicolumn{3}{c|}{\textbf{Structural measures}} & \multicolumn{5}{c}{\textbf{Semantic relatedness}} \\
    	

    	\multicolumn{2}{c|}{Model} & $\rho_{vis}$ & $C_{intra}$ & $C_{inter}$ & STS/All & STS/Cap. & STS/News &STS/For. & SICK \\
        \hline
Text-only & \textbf{ST}  &16 & 43& 25   & 40/41  & 44/42 & 38/42 & 21/22 &  52/55 \\ 
Projection \textbf{P} & $\textbf{P}^p(0)$ & 37 & 63 & 06  &  62/67 & 82/84& 43/48 & \textbf{29}/\textbf{31} & 61/75 \\ 
        \hline
Cluster $\textbf{M}_{cluster}$ &$ \textbf{M}^p(0,\phantom{.1}0,1)$ & 38 & \textbf{66} & \textbf{01}  & 62/66 & 83/84 & 41/46 & 22/24 & \textbf{62}/\textbf{76} \\ 
Perceptual $\textbf{M}_{perc}$ & $\textbf{M}^p(0,\phantom{0.}1,0)$ & \textbf{53} & 44 & 18  &58/60  & 75/75 & 41/45 & 23/26 & 59/63\\
Both combined $\textbf{M}_{both}$ & $\textbf{M}^p(0,0.1,1)$ & 46 & 63 & 02    & \textbf{64}/\textbf{68} & \textbf{84}/\textbf{85} & \textbf{44}/\textbf{49} & 27/29 & \textbf{62}/\textbf{76} \\ 
    \end{tabularx}
    \end{center}
    \vspace{-0.2cm}
    \caption{\textbf{RQ1,2}: (MSVD) Structural measures and semantic relatedness performances for different grounding hypotheses.}
    \label{vrep_M2}
\end{table*}

==> table_grounding_f.tex <==
\newlength{\ltwosmall}
\setlength{\ltwosmall}{25pt}

\begin{table*}[t]
\small
\begin{center}

\begin{tabularx}{\textwidth}{l l | C{\ltwosmall}  C{\ltwosmall} C{\ltwosmall}  C{\ltwosmall} | Y Y Y Y Y} \multicolumn{2}{r}{} &  \multicolumn{4}{c|}{\textbf{Structural measures}} & \multicolumn{5}{c}{\textbf{Semantic relatedness}} \\
\multicolumn{2}{c|}{Model} & $\mnno_{f(X)}$ & $\rho_{vis}$& $C_{inter}$ & $C_{intra}$ & STS/All & STS/Cap. & STS/News &STS/Forum & SICK  \\
\hline 
Textual & $\textbf{T}$ &10.0 & 4.1 & 54.2 & 70.1& 30 &41&36 &21 &51\\
Projection& \textbf{CM} & 27.1 & 19.2 & 1.5 & 85.8 & 56 & 78 & 40 & 34 & 55 \\ 
\hline 
Perceptual&$\textbf{P}_g$& 21.3& \textbf{32.4}& 43.9&73.3& 45&66&41&\textbf{37}&53\\ 
Cluster&$\textbf{C}_g$& 28.6 & 9.4&\textbf{1.1}& \textbf{88.5}& 62&83&46&29&59\\ 
Both&$\textbf{C}_g+\textbf{P}_g$& \textbf{28.9} & 29.1& 4.7&87.5& \textbf{63} &\textbf{84}& \textbf{48}&33&\textbf{60}\\

\end{tabularx}
\end{center}
\vspace{-0.2cm}
\caption{Intrinsic evaluations: comparison of various grounding hypotheses}
\vspace{-0.3cm}
\label{vrep_M2}
\end{table*}






==> table_motivation.tex <==
\newlength{\fsize}
%\setlength{\fsize}{7.59pt}
\setlength{\fsize}{9.2pt}
\newlength{\flsize}
\setlength{\flsize}{10pt}
\begin{table}[t]
    \begin{center}
    \begin{tabularx}{\textwidth}{l | c c c}
      %\hline
      \multicolumn{1}{c|}{Parameters} & \multicolumn{1}{c}{$(X,Y)$} & \multicolumn{1}{c}{$(X,f(X))$} &
      \multicolumn{1}{c}{$(Y,f(X))$} &
      \\

    $\{\theta, MLP \}$&  & &  \\
      $\{MLP\}$ & 10.0 & 15.1 &23.3\\ 
    \end{tabularx}
    \vspace{-0.1cm}
    \caption{mNNO values for projection baseline. Top row: retropropagation trough textual encoder.}
    \label{table_qualitative}
    \end{center}
    \vspace{-0.5cm}
\end{table}


==> word.tex <==

\newlength{\lword}
\setlength{\lword}{25pt}


\begin{table}[t]
    \begin{center}
    %\footnotesize
    
    
	\begin{tabularx}{\textwidth}{l | C{\lword} C{\lword} C{\lword} C{\lword} C{\lword} }	\multicolumn{1}{l|}{}  &  \rota{VisSim} & \rota{SemSim} & \rota{Simlex} & \rota{MEN}  & \rota{WordSim}\\


\textbf{T} & 47 & 60 & 45 & 60 & 57 \\
\textbf{M} & \textbf{52} & \textbf{64} & \textbf{49} & \textbf{67} & \textbf{59} \\

    \end{tabularx}
    \caption{Semantic relatedness scores on word representations}
   \vspace{-0.8cm}
    \label{words}
    \end{center}
\end{table}
